Molecular gas budget and characterization of intermediate-mass star-forming galaxies at $z\approx 2-3$

Star-forming galaxies (SFGs) with stellar masses below $10^{10}\,M_\odot$ make up the bulk of the galaxy population at $z>2$. The properties of the cold gas in these galaxies can only be probed in very deep ALMA observations or by targeting strongly lensed galaxies. Here we report the results of a pilot survey using the Atacama Compact Array (ACA) of molecular gas in the most strongly magnified galaxies selected as giant arcs in optical data. The selection in rest-frame UV wavelengths ensures that sources are regular star forming galaxies, without a priori indications of intense dusty starburst activity. We conducted Band 4 and Band 7 observations to detect mid-$J$ CO, [C I] and thermal continuum as molecular gas tracers from four strongly lensed systems at $z\approx2-3$: our targets are SGAS J1226651.3+215220 (A and B), SGAS J003341.5+024217 and the Sunburst Arc. The measured molecular mass is then projected onto the source plane with detailed lens models developed from high resolution HST observations. Multiwavelength photometry is then used to obtain the intrinsic stellar mass and star formation rate via SED fitting. In only one of the sources are the three tracers robustly detected, while in the others they are either undetected or detected in continuum only. The implied molecular gass masses range from $4\times 10^{9}\,M_\odot$ in the detected source to an upper limit of $\lesssim 10^9\,M_\odot$ in the most magnified source. The inferred gas fraction and gas depletion timescale are found to lie approximately 0.5 to 1.0 dex below the established scaling relations based on previous studies of unlensed massive galaxies. Our results indicate that the cold gas content of intermediate to low mass galaxies should not be extrapolated from the trends seen in more massive high-$z$ galaxies. (Abridged abstract)

==> hst_obs.tex <==
% PSZG311 field: ACS/F814W, WFC3/F275W --> (PI: Dahle, H., prop:) WFC3/F606W, WFC3/F160W --> (PI: Bayliss, M., prop:)
% SGASJ1226 field: WFC3/F606W,  WFC3/F814W --> (PI: Morris, G., prop:), WFC3/F110W, WFC3/F160W --> (PI: Bayliss, M., prop:)
% SGASJ0033 field: WFC3/F555W, WFC3/F814W, WFC3/F110W, WFC3/F140W --> (PI: Wuyts, E., prop:) 
\begin{tabular}{c|rlcccc}
    \hline\hline
     Field & Instrument & Filter & $\lambda_\text{pivot}^\text{rest}$ (\si{\micro\meter}) & $t_\text{exp}$ (s) & Program ID \\
     \hline
     \multirow{3}*{PSZ1 G311.65-18.48} & ACS WFC & F814W &  0.238 & 5280 & GO15101 (PI: Dahle) \\
     \cline{2-6}
                                         & WFC3 UVIS & F606W & 0.175 & 1484 & \multirow{2}*{GO15377 (PI: Bayliss)} \\
                                         & WFC3 IR & F160W & 0.456 & 1359 & \\
     \hline
     \multirow{4}*{SGAS J122651.3+215220} & ACS WFC & F814W & 0.205 & 2040 & \multirow{2}*{GO12368 (PI: Morris)} \\
                                            & ACS WFC & F606W & 0.151 & 2040 &  \\
                                            \cline{2-6}
                                            & WFC3 IR & F110W & 0.294 & 1212 & \multirow{2}*{GO15378 (PI: Bayliss)} \\
                                            & WFC3 IR & F160W & 0.392 & 1312 & \\
    \hline
    \multirow{4}*{SGAS J003341.5+024217} & WFC3 UVIS & F555W & 0.157 & 1748 & \multirow{4}*{GO14170 (PI: Wuyts)} \\
                                           & WFC3 UVIS & F814W & 0.237 & 1900 & \\
                                           & WFC3 IR & F105W & 0.311 & 721 & \\
                                           & WFC3 IR & F140W & 0.411 & 459 &  \\
    \hline\hline
\end{tabular}
